Language acquisition: do children and language models follow similar learning stages?

During language acquisition, children follow a typical sequence of learning stages, whereby they first learn to categorize phonemes before they develop their lexicon and eventually master increasingly complex syntactic structures. However, the computational principles that lead to this learning trajectory remain largely unknown. To investigate this, we here compare the learning trajectories of deep language models to those of children. Specifically, we test whether, during its training, GPT-2 exhibits stages of language acquisition comparable to those observed in children aged between 18 months and 6 years. For this, we train 48 GPT-2 models from scratch and evaluate their syntactic and semantic abilities at each training step, using 96 probes curated from the BLiMP, Zorro and BIG-Bench benchmarks. We then compare these evaluations with the behavior of 54 children during language production. Our analyses reveal three main findings. First, similarly to children, the language models tend to learn linguistic skills in a systematic order. Second, this learning scheme is parallel: the language tasks that are learned last improve from the very first training steps. Third, some - but not all - learning stages are shared between children and these language models. Overall, these results shed new light on the principles of language acquisition, and highlight important divergences in how humans and modern algorithms learn to process natural language.

==> 11_abtract_linnea.tex <==

% general goal
% the challenge
% why your method tackle this challenge
% results
% the conclusion: why it matters

% We suggest 3 hypotheses regarding the stages of language acquisition. The first hypothesis is that there are no stages; all linguistic phenomena are learned at the same time. The second hypothesis is that linguistic phenomena are learned sequentially but the order of that sequence is different per agent. The final hypothesis is that linguistic phenomena are necessarily learned in the same order by all language agents.


Three distinct stages have been observed in children's language acquisition, in which all linguistic phenomena in the first stage must be exhibited before phenomena in the second stage can be exhibited and so on; however, the learning dynamics behind these stages are unobservable. To investigate this, we study whether artificial neural networks, which are fully observable, have the same stages in language acquisition as children by using behavioural linguistic probes, and what the learning dynamics of these networks are.

We suggest two hypotheses regarding learning dynamics. The first hypothesis is that children learn linguistic phenomena sequentially: they cannot start learning the next stage until the previous stage is fully learned. The second hypothesis is that a child learns all linguistic phenomena in parallel, but phenomena in the subsequent stage are only fully acquired (and thus observable in the child) after the current stage is complete.

We found that GPT-2 networks learn all linguistic phenomena in parallel from the start of training. The order in which these phenomena are fully acquired is the same across all random seeds, with p value < 0.001. The stages learned by the networks correlate to the stages observed in children with r value = 0.579.

Our results suggest that artificial neural networks do learn linguistic tasks in the same order as children, however, as the linguistic tests for artificial neural networks are not exactly the same as those used to evaluate children we highlight that further work is required to develop appropriate tests. From this body of work we conclude that neural networks learned tasks in a fixed order and in parallel, and suggest that the discrete stages in language acquisition observed in children may be an artifact of the granularity of the language evaluations and may be better explained by continuous and parallel learning dynamics.


% Conclusion: it was hard to find something theory driven but it was possible to find the learning trajectory data driven.

% Theory driven clustering vs data driven clustering.

==> remove.tex <==

@article{babyberta_zorro,
Current file
Overview
Drop Argument
Animate Subject Trans
Filler-Gap-Wh Question Subject
Existential There Quantifiers 1
Principle A Case 1
Case-Subjective Pronoun
Sentential Negation Npi Licensor Present
Tough Vs Raising 2
Passive 2
Wh Questions Subject Gap
Wh Questions Subject Gap Long Distance
Wh Vs That No Gap
Wh Vs That No Gap Long Distance
Expletive It Object Raising
Argument Structure-Swapped Arguments
Animate Subject Passive
Existential There Object Raising
Principle A Domain 1
Filler-Gap-Wh Question Object
Irregular-Verb
Irregular Past Participle Verbs
Argument Structure-Transitive
Quantifiers-Superlative
Passive 1
Left Branch Island Echo Question
Regular Plural Subject Verb Agreement 1
Transitive
Island-Effects-Coordinate Structure Constraint
Agreement Subject Verb-Across Prepositional Phrase
Anaphor Number Agreement
Agreement Determiner Noun-Across 1 Adjective
Agreement Subject Verb-In Simple Question
Argument Structure-Dropped Argument
Determiner Noun Agreement Irregular 2
Determiner Noun Agreement 1
Determiner Noun Agreement 2
Anaphor Agreement-Pronoun Gender
Short Nested Inner
Quantifiers-Existential There
Binding-Principle A
Regular Plural Subject Verb Agreement 2
Determiner Noun Agreement Irregular 1
Determiner Noun Agreement With Adjective 1
Coordinate Structure Constraint Object Extraction
Npi Licensing-Only Npi Licensor
Principle A Domain 2
Long Nested Inner
Determiner Noun Agreement With Adj Irregular 2
Irregular Plural Subject Verb Agreement 1
Agreement Subject Verb-Across Relative Clause
Causative
Irregular Past Participle Adjectives
Determiner Noun Agreement With Adj Irregular 1
Long Nested Outer
Determiner Noun Agreement With Adj 2
Existential There Subject Raising
Short Nested Outer
Nounpp
Simple
Principle A Case 2
Ellipsis N Bar 2
Irregular Plural Subject Verb Agreement 2
Distractor Agreement Relational Noun
Ellipsis-N Bar
Correct Example Incorrect ExampleLinguistic Test
The Lutherans couldn't skate around. The Lutherans couldn't disagree with.
Danielle visited Irene. The eye visited Irene.
Chris reached the bear that is washing trains. Chris reached who the bear is washing trains.
There aren't many lights darkening. There aren't all lights darkening.
Tara thinks that she sounded like Wayne. Tara thinks that herself sounded like Wayne.
They gave the person the tour. The person gave they the tour.
Those banks had not ever lied. Those banks had really ever lied.
Rachel was apt to talk to Alicia. Rachel was exciting to talk to Alicia.
Most cashiers are disliked. Most cashiers are flirted.
Cheryl thought about some dog that upset Sandra. Cheryl thought about who some dog upset Sandra.
Bruce knows that person that Dawn likes that argued about a lot of guys. Bruce knows who that person that Dawn likes argued about a lot of guys.
Danielle finds out that many organizations have alarmed Chad. Danielle finds out who many organizations have alarmed Chad.
Christina forgot that all plays that win worry Dana. Christina forgot who all plays that win worry Dana.
Regina wanted it to be obvious that Maria thought about Anna. Regina forced it to be obvious that Maria thought about Anna.
They built the mouse that farm. The mouse built that farm they.
Amanda was respected by some waitresses. Amanda was respected by some picture.
William has declared there to be no guests getting fired. William has obliged there to be no guests getting fired.
Carlos said that Lori helped him. Carlos said that Lori helped himself.
Laura got the suit that the bird cut. Laura got what the suit cut the bird.
Sarah spoke without thinking last night. Sarah spoken without thinking last night.
Edward hid the cats. Edward hidden the cats.
Will robert eat? Will robert force?
No bird could catch more than six plants. No bird could catch at least six plants.
Jeffrey's sons are insulted by Tina's supervisor. Jeffrey's sons are smiled by Tina's supervisor.
David would cure what snake? What would David cure snake?
Jeffrey hasn't criticized Donald. Jeffrey haven't criticized Donald.
A lot of actresses' nieces have toured that art gallery. A lot of actresses' nieces have coped that art gallery.
What did sarah and the person work for? What did sarah work for and the person?
The brother by the lion is red. The brothers by the lion is red.
Many teenagers were helping themselves. Many teenagers were helping herself.
Look at this happy piece. Look at this happy pieces.
What color was the piece? What color was the pieces?
My brother moves fast. My brother moves to.
Those ladies walk through those oases. Those ladies walk through that oases
Craig explored that grocery store. Craig explored that grocery stores.
Carl cures those horses. Carl cures that horses.
She will give herself the wire. She will give himself the wire.
The actor that the boy attracts. The actor that the boy attract.
There was a leg that anne made. There was most leg that anne made.
Sarah thinks about herself making a tree. Sarah thinks about herself makes a tree.
The dress crumples. The dresses crumples.
Phillip was lifting this mouse. Phillip was lifting this mice.
Tracy praises those lucky guys. Tracy praises those lucky guys.
Who will Elizabeth and Gregory cure? Who will Elizabeth cure and Gregory?
Only his rabbit will ever be in her magic. Even his rabbit will ever be in her magic.
Mark imagines Erin might admire herself. Mark imagines Erin might admire himself.
The actor that the boy beside the woman attracts. The actor that the boy beside the woman attract.
That adult has brought that purple octopus. That adult has brought those purple octopus.
This goose isn't bothering Edward. This goose weren't bothering Edward.
The pages that i like were dirty. The page that i like were dirty.
Aaron breaks the glass Aaron appeared the glass.
Edward hid the cats. Edward hidden the cats.
This person shouldn't criticize this upset child. This person shouldn't criticize this upset children.
The actor that the boy beside the woman attracts greets. The actor that the boy beside the woman attracts greet.
Some actors buy these gray books. Some actors buy this gray books.
There was bound to be a fish escaping. There was unable to be a fish escaping.
The actor that the boy attracts blocks. The actor that the boy attracts block.
The athlete behind the bike approves. The athlete behind the bike approve.
The athlete admires. The athlete admire.
Stacy imagines herself praising this actress. Stacy imagines herself praises this actress.
Curtis's boss discussed four sons and Andrew discussed five sick sons. Curtis's boss discussed four happy sons and Andrew discussed five sick.
The woman cleans every public park. The women cleans every public park.
A sketch of lights doesn't appear. A sketch of lights don't appear.
Allen got one roman brain and chris got two. Allen got one brain and chris got two roman.
0 2000 4000 6000 8000 10000 12000 14000
Training Step
Steps to Reach 90% of Final AccuracyFigure 2: Linguistic tests used to probe the artificial neural networks. Training curves are smoothed using a moving
average filter with window size of 6 checkpoints then the number of steps required to reach 90% of final accuracy is
calculated. Tests are ordered by increasing number of steps on average. Results shown for 48 runs. Only tests which
have final accuracy greater than chance (50%) are shown. This demonstrates that tests are learned in the same order
by all agents, disproving the null hypothesis.
4
3.1 Learning is parallel across linguistic tasks2300 2000 4000 6000 8000 10000 12000 14000 16000
Training Step
40
50
60
70
80
90
Accuracy (%)
Chance Level
DNN Performance on 3 Groups of Linguistic Tests
Stage 1
Stage 2
Stage 3
Tests not Learned
Figure 3: Linguistic tests used to probe the artificial
neural networks grouped into 3 groups to avoid plotting
one line per linguistic test. Tests which have final ac-
curacy less than chance (50%) are place in their own
group). Shading is standard error of the mean across
tests in the stage. This demonstrates that linguistic skills
are learned in parallel not in sequence. The tests in each
group correspond to the colours in Figure 2.
Are these linguistic skills learned sequentially or231
in parallel? To address this question, we group the232
64 tests into three groups according to their average233
acquisition time (Figure 2).234
Figure 3 presents the mean accuracy during train-235
ing for each group, averaged across tests and ran-236
dom seeds. To formally compare the learning tra-237
jectory of these three groups, we identify, for each238
random seed, where the average performance ob-239
tained in a given group begins rising, (i.e. where240
the derivative of the learning curve is greater than a241
threshold). We perform a one-way ANOVA test on242
the training steps necessary to reach this threshold243
for each stage, for all random seeds. The results are244
significant (p < 1.e-36) for all gradient thresholds245
between 0 and 20 indicating that learning begins at246
a different time for each of the 3 stages, it does not247
all start from the beginning of training.248
3.2 Comparison with children249
We compare 3 probes on our models to 3 linguis-250
tic phenomena quantified in two- to six-year old251
children by (Friedmann et al., 2021). (Friedmann252
et al., 2021) shows that there are three stages in chil-253
dren’s language acquisition (here shown in green,254
blue and red in Figure 4). The first stage is marked255
by simple subject-verb agreement, the second low256
CP zone structures, and the third by high CP zone 257
structures. There is a clear order in which the stages 258
are acquired, first, second then third, in both the 259
children and our models. We do not quantify the 260
correlation between the children and models as it 261
would be based on only three linguistic probes. 262
3.3 Detailed analysis of syntax acquisition 263
We first grouped our probes into 3 stages empir- 264
ically (Section 3.1), now we examine the three 265
stages defined linguistically by (Friedmann et al., 266
2021) to determine whether the stages are learned 267
in sequence or in parallel. Learning of all three 268
stages is in parallel and reaches above chance level 269
(Figure 5a). 270
To determine whether our models are truly learn- 271
ing syntax we examine three probes which can be 272
split into congruent and incongruent cases. Incon- 273
gruent cases are the most difficult and require real 274
knowledge of the syntax of the sentence. The mod- 275
els do not learn stage 3 above chance level, and just 276
barely reach chance level on stage 2 (Figure 5b), 277
indicating that they are using some grammatical 278
short cuts to achieve high accuracy on the congru- 279
ent cases (leading to above chance performance on 280
the probe overall Figure 5a) and lack real under- 281
standing of syntax. On the contrary, the pretrained 282
GPT-2 large achieved above 75% accuracy on even 283
the incongruent cases of these probes. 284
Previous work (Ref??) suggests that artificial 285
neural networks may have a bias towards the plu- 286
ral form of verbs in English, as plural verbs are 287
shorter than singular verbs (consider "they run" vs 288
"he runs"), meaning they often consist of a single 289
token while singular verbs will be split into two 290
tokens. Since the probability of one token followed 291
by another is the product of the probabilities of 292
each word, the combined probability of the two 293
will always be lower than the probability of a sin- 294
gle token, hence leading to the bias towards shorter 295
words, the plural form in English. 296
To examine whether bias has a significant effect 297
on our analysis we look at the difference in model 298
performance on sentences with only singular or 299
only plural verbs, as well as congruent and incon- 300
gruent cases. Accuracy on predicting plural verbs 301
increases sharply from the start of the training and 302
then falls. By contrast, the accuracy of singular 303
cases falls first and then rises (Figure 5c) 304
This offers an explanation of the sharp rise then 305
decline of "Left Branch Island Simple Question" 306
5
18 22 22 23 23 23 24 24 25 26 29 30 32 35 35 36 37 38 39 41 48 53 58 59 62 64 68 70
Age (months)
Sv Simple
Wh Adjunct Excl Why
Relative Clause
Linguistic Test Linguistic Stages in Children
The boy built a tower
What sound does a cow make?
I will take another shape that I want
Observed Examples
0
600
1200
1800
2400
3000
3600
4200
4800
5400
6000
6600
7200
7800
8400
9000
9600
10200
10800
11400
12000
12600
13200
13800
14400
15000
15600
Training Step
Subject Verb Agreement
Agreement Subject Verb-In Simple Question
Short Nested Outer
Linguistic Test Linguistic Stages in Artificial Neural Networks
This goose isn′t bothering Edward
What color was the piece?
The actor that the boy attracts blocks
Correct Example
This goose weren′t bothering Edward
What color was the pieces?
The actor that the boy attracts block
Incorrect Example
Stage 1
Stage 2
Stage 3Figure 4: Comparing ANN performance on linguistic tests to children’s performance. Example sentences observed
in children were originally in Hebrew (Friedmann et al., 2021). Non-white indicates the phenomena is learned by
the agent. The threshold for considering a test learned for the ANN is performance above 55%.0 2000 4000 6000 8000 10000120001400016000
Training Step
50
60
70
80
90
Accuracy (%)
Chance
Subject Verb Agreement
Simple
Nounpp
Agreement Subject Verb-In Simple Question
Short Nested Outer
(a)0 2000 4000 6000 8000 10000120001400016000
Training Step
20
40
60
80
Accuracy (%)
Chance
Subject Verb Agreement on Incongruent Cases
Simple Singular
Nounpp Singular Plural
Short Nested Outer Singular Plural (b)0 2500 5000 7500 10000 12500 15000
Training Step
20
40
60
80
Accuracy (%)
Subject Verb Agreement: Simple
Plural Singular
0 2500 5000 7500 10000 12500 15000
Training Step
20
40
60
80
Subject Verb Agreement: NounPP
Singular Singular
Singular Plural
Plural Singular
Plural Plural
0 2500 5000 7500 10000 12500 15000
Training Step
20
40
60
80
Subject Verb Agreement: Short Nested Outer
Singular Singular
Singular Plural
Plural Singular
Plural Plural
(c)
Figure 5: Subject verb agreement. Shading is standard error of the mean across seeds. (a) Parallel learning is
observed in the three stages defined by (Friedmann et al., 2021). (b) Subject verb agreement on incongruent cases
which are most difficult for the models and indicate whether the model understands syntax. The networks do not
learn some syntax structures as the incongruent case of Short Nested Outer does not reach above chance level here.
(c) The models are biased towards plural rather than singular as a result of tokenization.
6
in Figure ??. We note that when averaging over307
the congruent and incongruent cases the biases are308
accounted for as shown in Figure 5a.309
MISSING SECTION CONCLUSION HERE:310
what do you retain from all these syntactic analy-311
ses? what’s the 1-line summary of the comparison312
between children and models in terms of syntax?313
4 Discussion314
The stages followed by children to acquire lan-315
guage has been the topic of an intense research.316
While, this learning trajectory is becoming clearer317
for sub-lexical representations, the acquisition of318
higher-level processing remains more parsimo-319
nious. Here we approach this historical question320
through the lens of the deep language models.321
These artificial neural networks, trained to predict322
words from context, have proved to323
Firstly, we show that deep models learn linguis-324
tic phenomena in the same order across random325
seed with p < 0.001. Recent studies have shown326
that transformer models can learn grammar from327
the limited vocabulary present in child-directed cor-328
pora (Huebner et al., 2021) and have demonstrated329
the presence of syntax in deep net representations330
(Lakretz et al., 2019; Linzen et al., 2016), but have331
not examined how these abilities develop during332
training or the order in which they are acquired,333
which is our unique contribution.334
Secondly, we demonstrate that linguistic abil-335
ities are learned in parallel, meaning that harder336
tasks are learned at the same time as easier tasks337
but at a slower rate. However, we note that our338
hypothesis of either sequential or parallel learning339
was overly simplistic, as we observe that the hard-340
est tests, shown in the red line in Figure 3, do not341
start increasing in accuracy from the beginning of342
training (and we showed the 3 stages have statisti-343
cally different times at which learning starts). This344
resembles a mix of sequential and parallel learning345
as there is a delay before performance on the hard-346
est tests improves, but still they improve before347
the easier group, the blue line, has reached its final348
accuracy. This is builds upon previous results that349
showed the learning dynamics of children to be dis-350
crete stages (Friedmann et al., 2021). We argue that351
the discrete stages shown in children are a result of352
the granularity of probing. As it is easy to probe353
deep nets at very small increments during training,354
we can observe the parallel learning dynamics that355
are likely present in children as well but difficult to356
probe. 357
Finally, we show that there is a significant cor- 358
relation (r = 0.579, p < XX) between the stages in 359
deep nets’ and children’s acquisition. These stages 360
are defined in terms of linguistic theory derived 361
from observation of children. This is complemen- 362
tary to a recent study which showed that the rep- 363
resentations of artificial neural networks become 364
increasingly similar to the representations of the 365
adult brain during training (Caucheteux and King, 366
2022). Our analysis is on linguistic probes which 367
relate directly to linguistic theory rather than on 368
internal brain and deep net representations. 369
We present the issue of biases towards the plural 370
form of words in our model in Figure 5c. This 371
could an effect of tokenization as plural nouns in 372
English are systematically shorter than singular 373
nouns (consider "he runs" vs "they run"). In the 374
standard GPT-2 tokenizer used here, singular verbs 375
can be split into multiple tokens ([run] [s]) where 376
a plural verb remains one ([run]). Since the prob- 377
ability of two tokens occurring in succession is 378
lower than a single token, the likelihood of singular 379
verbs is biased to be lower. We note that this issue 380
could be solved by training the model on a larger 381
dataset, as while our models learn only 66% of 382
tasks to above chance level, OpenAI GPT-2 learns 383
97%. OpenAI GPT-2 was trained on 40GB of data, 384
while our model was trained on only 500 MB. Both 385
the issues of biases towards plural verbs and tests 386
not learned above chance level could be solved by 387
training on a larger dataset. Another limitation of 388
this study is the mismatch between our probes and 389
those used for analysing children. 390
The conclusion that the language stages in deep 391
nets correlate to those in children should be ex- 392
tended to the speech domain for a more realis- 393
tic comparison. This could be done by probing 394
a model such as Wav2Vec (Baevski et al., 2020). 395
For this analysis the same probes could be used in 396
speech form, however this leads to a comment on 397
the suitability of the linguistic probe corpora avail- 398
able. We find that many of the probes designed 399
to test a given phenomenon also inadvertently test 400
for others, thus if a model does not pass a given 401
test it may be that the probes need to be designed 402
suitably. 403
In particular the probes which we matched to 404
the data on children were not identical to the phe- 405
nomena observed in children. However, even if 406
the phenomena matched perfectly the method of 407
7
testing for the deep nets and children was differ-408
ent. The children were observed producing a phe-409
nomenon while the deep nets were asked whether410
they understood which sentence was correct. As411
GPT-2 has been designed to produce language it412
could be interesting to examine whether it would413
produce the correct next word given an input sen-414
tence. However to be truly comparable to children,415
this would require stimulus with a context not stand416
alone sentences.417
Our results have implications for the field of ma-418
chine learning as now that it is evident that deep419
nets learn in the same order as children, the main is-420
sue left to solve is the relatively enormous amount421
of data they require to learn. For developmental422
psychology we suggest that deep nets are used as a423
model to probe incremental learning dynamics that424
are difficult to measure in children due to practical425
constraints, and point out that certain staircase-like426
results in children may be a result of granularity of427
measurement rather than real jumps in understand-428
ing.429
Acknowledgements430
References431
Alexei Baevski, Henry Zhou, Abdelrahman Mohamed,432
and Michael Auli. 2020. wav2vec 2.0: A frame-433
work for self-supervised learning of speech rep-434
resentations. Advances in Neural Information435
Processing Systems, 2020-Decem:1–12. Under-436
stand wav2vec 2.0:<br/><br/>Use convolution then437
quot;discretisequot; to get distinct features. Then ob-438
scure certain features at some timesteps (for self-439
supervision). Then use transformers to learn a predict440
those obscured parts.<br/>Works well even on 10441
mins of unlabelled data. Can be fine tuned with a442
small amout of labelled data (labels phonemes in that443
language for example).444
Charlotte Caucheteux and Jean Rémi King. 2022.445
Brains and algorithms partially converge in natural446
language processing. Communications Biology, 5(1).447
Naama Friedmann, Adriana Belletti, and Luigi Rizzi.448
2021. Growing trees: The acquisition of the left449
periphery. Glossa: a journal of general linguistics,450
39(1).451
Kristina Gulordava, Piotr Bojanowski, Edouard Grave,452
Tal Linzen, and Marco Baroni. 2018. Colorless green453
recurrent networks dream hierarchically. In Proceed-454
ings of the 2018 Conference of the North American455
Chapter of the Association for Computational Lin-456
guistics: Human Language Technologies, Volume457
1 (Long Papers), pages 1195–1205, New Orleans,458
Louisiana. Association for Computational Linguis-459
tics.460
Philip Huebner. 2022. Unmasked. https:// 461
github.com/phueb/UnMasked. 462
Philip A Huebner, Elior Sulem, Cynthia Fisher, and Dan 463
Roth. 2021. BabyBERTa : Learning More Grammar 464
With Small-Scale Child-Directed Language. Pro- 465
ceedings of the 25th Conference on Computational 466
Natural Language Learning, pages 624–646. 467
Yair Lakretz, Dieuwke Hupkes, Alessandra Vergallito, 468
Marco Marelli, Marco Baroni, and Stanislas Dehaene. 469
2021. Mechanisms for handling nested dependen- 470
cies in neural-network language models and humans. 471
Cognition, 213:104699. Special Issue in Honour of 472
Jacques Mehler, Cognition’s founding editor. 473
Yair Lakretz, German Kruszewski, Theo Desbordes, 474
Dieuwke Hupkes, Stanislas Dehaene, and Marco Ba- 475
roni. 2019. The emergence of number and syntax 476
units in LSTM language models. In Proceedings of 477
the 2019 Conference of the North American Chap- 478
ter of the Association for Computational Linguistics: 479
Human Language Technologies, Volume 1 (Long and 480
Short Papers), pages 11–20, Minneapolis, Minnesota. 481
Association for Computational Linguistics. 482
Tal Linzen, Emmanuel Dupoux, and Yoav Goldberg. 483
2016. Assessing the Ability of LSTMs to Learn 484
Syntax-Sensitive Dependencies. Transactions of the 485
Association for Computational Linguistics, 4:521– 486
535. 487
Jacques Mehler, Peter Jusczyk, Ghislaine Lambertz, 488
Nilofar Halsted, Josiane Bertoncini, and Claudine 489
Amiel-Tison. 1988. A precursor of language acquisi- 490
tion in young infants. Cognition, 29:143–178. 491
Stephen Merity, Caiming Xiong, James Bradbury, and 492
Richard Socher. 2016. Pointer sentinel mixture mod- 493
els. 494
Alec Radford, Jeffrey Wu, Rewon Child, David Luan, 495
Dario Amodei, and Ilya Sutskever. Language Models 496
are Unsupervised Multitask Learners. 497
Alex Wang, Ian F. Tenney, Yada Pruksachatkun, 498
Katherin Yu, Jan Hula, Patrick Xia, Raghu Pappa- 499
gari, Shuning Jin, R. Thomas McCoy, Roma Patel, 500
Yinghui Huang, Jason Phang, Edouard Grave, Na- 501
joung Kim, Phu Mon Htut, Thibault F’evry, Berlin 502
Chen, Nikita Nangia, Haokun Liu, Anhad Mo- 503
hananey, Shikha Bordia, Nicolas Patry, Ellie Pavlick, 504
and Samuel R. Bowman. 2019. jiant 1.1: A soft- 505
ware toolkit for research on general-purpose text un- 506
derstanding models. http://jiant.info/. 507
Alex Warstadt, Alicia Parrish, Haokun Liu, Anhad Mo- 508
hananey, Wei Peng, Sheng Fu Wang, and Samuel R. 509
Bowman. 2020. Erratum: “blimp: The benchmark of 510
linguistic minimal pairs for english”. Transactions of 511
the Association for Computational Linguistics, 8:867– 512
868. 513
8

abstract = {Transformer-based language models have taken the NLP world by storm. However, their potential for addressing important questions in language acquisition research has been largely ignored. In this work, we examined the grammatical knowledge of RoBERTa (Liu et al., 2019) when trained on a 5M word corpus of language acquisition data to simulate the input available to children between the ages 1 and 6. Using the behavioral probing paradigm, we found that a smaller version of RoBERTa-base that never predicts unmasked tokens, which we term BabyBERTa, acquires grammatical knowledge comparable to that of pre-trained RoBERTa-base-and does so with approximately 15X fewer parameters and 6,000X fewer words. We discuss implications for building more efficient models and the learnability of grammar from input available to children. Lastly, to support research on this front, we release our novel grammar test suite that is compatible with the small vocabulary of child-directed input.},
author = {Huebner, Philip A and Sulem, Elior and Fisher, Cynthia and Roth, Dan},
file = {:C$\backslash$:/Users/linne/OneDrive/PhD/Papers Intro/FAIR/BabyBERTa.pdf:pdf},
journal = {Proceedings of the 25th Conference on Computational Natural Language Learning},
mendeley-groups = {FAIR},
pages = {624--646},
title = {{BabyBERTa : Learning More Grammar With Small-Scale Child-Directed Language}},
url = {https://github.com/huggingface/tokenizers},
year = {2021}
}

==> todo.tex <==
clean jargon: 
    2 hypotheses: sequential learning vs parallel learning
    1 architecture (GPT2
    48 models, (i.e. not agents)
    3 benchmark (i.e. not corpus, to be kept for wiki103)
    96 linguistic tests (i.e. not task, phenomenon, skill etc). Keep 'zero-shot probe' in method and 'language ability' in intro/discussion. 
    
    group:
       i) defined by linguists
       ii) defined empirically in our models
    training time: moment at which a test is achieve above threshold

clarify threshold definition

figure hypothesis: very clear, I also like the distinction between the three children, good job!
    - null hypothesis first
    - 'skill acquired' acquisition threshold -> in caption mention that it is partly arbitrary, but given the sigmoidal assumption, it does not have an impact
    - I'm wondering whether we shouldnt use a broken linear function, instead of a sigmoid (since the sigmoid always increases, even the sequential 
    - age of children -> + showing this behavior
    - training step -> '' (already have age of children below)
    - add chance level dotted line
    - remove vertical gray line


figure all tests:
    linguistic test: same line, no bold
    dots: maybe on log axis?
    'step to reach 90\% of final accuracy' -> acquisition time

figure children comparison: 
   - make matrix much narrower to gain width
   - order children by age?

figures: 
    add chance level
    remove top and right axis (ax.spines=['top'].set_visible(False)
    add caption
    specity what the error bar refer to
    try with a log training axis?
    
 
JR questions:
- why gray test below chance?
- shall we ask Dieuwke to interact with you to 1/ relaunch your script with wiki300Gb and 2/ relaunch it with OPT? I suspect that this first submission won't get easy because of our relatively poor performances, but it'll help us identify what the reviewers typically ask on this topic
    
Discussion
 - modest performance: finaly accuracy, small corpus
 - abritrary threshold: necessary as nearly non of the task achieve 90\% accuracy
 
 - biases
